Trends of Papers Published from 2006 to 2010 in Journals Nature and Science

We present an analysis of the papers published in the journals Nature and Science in the years from 2006 to 2010. During this period, a total of 7788 papers were published in the two journals. This includes 544 astronomy papers that comprise 7.0% of the papers in `all' research fields and 18.9% of those in the fields of `physical sciences'. The sub-fields of research of the astronomy papers are distributed, in descending order of number of papers, in Solar System, stellar astronomy, galaxies and the universe, the Milky Way Galaxy, and exoplanets. The observational facilities used for the studies are mainly ground-based telescopes (31.1%), spacecrafts (27.0%), and space telescopes (22.8%), while 16.0% of papers did not use any noticeable facilities and 1.7% used other facilities. Korean scientists have published 86 papers (33 in Nature and 53 in Science), which is 1.10% of all the papers (N=7788) in the two journals. The share of papers by Korean astronomers among the scientific papers by Koreans is 8.14%, slightly higher than the contribution of astronomy papers (7.0%) in both journals.

==> hfont.tex <==
%%% file `hfont.tex` ( a part of ko.TeX )
%%
%% (C) Copyright 2007 Koaunghi Un <koaunghi@kornet.net>
%%                    Dohyun Kim  <nomos@ktug.or.kr>
%%                    Kangsoo Kim <karnes@ktug.or.kr>
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3c
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%  http://www.latex-project.org/lppl.txt
%% and version 1.3c or later is part of all distributions of LaTeX
%% version 2006/05/20 or later.
%%
%% Read LICENSE included in the package.
%%
%% ------------------------------------------
%%
%% 이 파일은 우리말을 \TeX에서 사용하는데 필요한 KS X 1001 부호와
%% 글자체 정의에 그 역할을 두고 있다.  우리말 글자체는 \LaTeX2e의
%% NFSS2(New Font Selection Scheme2)을 한글화한 HFSS에 의해 선택되며,
%% 일반의 한글문서와는 달리 문서에 우리말 글자체만 포함하기 위해서는
%% 이 파일이 단독으로 사용될 수 있다.
\ProvidesFile{hfont.tex}[2007/07/15]

%% 0.95 scheme

\begingroup
\def\reserved@a{}\count@="0A1
\loop\ifnum\count@<\@cclvi
  \edef\reserved@a{\reserved@a \sfcode\the\count@=\@m}%
  \advance\count@ by1
\repeat
\global\let\ks@break\reserved@a
\endgroup

%% 우리말 부호의 정의 (KSC5601)
%% ----------------------------
%% 우리말부호는 모두 TeX의 모듬명령으로 처리된다.
\def\reserved@a#1#2{%
  \@tempcnta#1\relax
  \@tempcntb#2\relax
  \reserved@b}
\def\reserved@b{%
  \ifnum\@tempcnta>\@tempcntb\else
    \reserved@c\@tempcnta
    \advance\@tempcnta\@ne
    \expandafter\reserved@b
  \fi}
\def\reserved@c#1{%
  \uccode#1=#1
  \lccode#1=#1
  \sfcode#1=1001
  \catcode#1=\active}
\reserved@a{"0A1}{"0FE}

\begingroup
\def\ksc@code{\ifnum\count@<"0FF
  \edef\reserved@a{\reserved@a \catcode\the\count@=\the\@tempcnta}
  \advance\count@ by1
  \else\let\next\relax \fi\next}
\@tempcnta13
\def\reserved@a{}\count@="0A1\let\next\ksc@code \ksc@code
\global\let\makekscactive\reserved@a
\@tempcnta12
\def\reserved@a{}\count@="0A1\let\next\ksc@code \ksc@code
\global\let\makekscother\reserved@a
\@tempcnta11
\def\reserved@a{}\count@="0A1\let\next\ksc@code \ksc@code
\global\let\makekscletter\reserved@a
\endgroup

%% 우리말의 분철:
%% --------------
%% 우리말은 \hyphenchar가 없고 어느 곳에서나 分綴이 可能하다. 그러므로
%% 일단 글자체 자체에서 分綴을 억제하고 (\hyphenchar\font\m@ne)
%% 우리말 사이에 \hskip\hangul@skip을 揷入함으로써 分綴을 可能하게
%% 함과 동시에 \hangulskip으로 자간간격을 조절을 할 수 있도록 한다.
%%
\newdimen\hangulskip
\newskip\hangul@skip
\def\@Hyphen{\ifhmode\ifnum\spacefactor=1001\hskip\hangul@skip\fi\fi}%%%%
\def\set@hangulskip{%
  \@tempdima=\f@size\p@
  \multiply\@tempdima100
  \divide\@tempdima\p@
  \multiply\@tempdima\p@
  \hangul@skip=\hangulskip minus\hangulskip
  \multiply\hangul@skip by\strip@pt\@tempdima%
  \divide\hangul@skip by1000
}

%% 줄바꿈의 억제
% 우리말 음절은 어느 곳에서든지 줄바꿈이 가능하다.  줄바꿈을 억제할
% 때에 라텍의 \nolinebreak도 효과가 없다.  우리말 음절의 경계에서는
% 다음과 같이 줄바꿈을 억제한다.
\def\noHyphen{\spacefactor=999\nolinebreak}

%% 우리말의 글자체 바꾸기:
%% -----------------------
%% 우리말의 글자체종류는 명조와 고딕 그리고 타자의 3가지를 기본으로
%% 한다. 명조(\textmj)와 고딕(\textgt)은 각각 영문의 \textrm과
%% \textsf에 해당하고 타자(\texttz)는 영문의 \texttt와 같다.
\DeclareTextFontCommand{\textmj}{\mjfamily}
\DeclareTextFontCommand{\textgt}{\gtfamily}
\DeclareTextFontCommand{\texttz}{\tzfamily}

%% 우리말글자체가족은 명조, 고딕, 타자의 세가지가 있고 다음과 같은
%% 등식이 성립한다. \rmfamily=명조, \sffamily=고딕, \ttfamily=타자.
\expandafter\def\expandafter\rmfamily\expandafter{\rmfamily
         \not@math@alphabet\mjfamily\mathmj
         \hfontfamily\mjdefault}
\let\mjfamily\rmfamily
\expandafter\def\expandafter\sffamily\expandafter{\sffamily
         \not@math@alphabet\gtfamily\mathgt
         \hfontfamily\gtdefault}
\let\gtfamily\sffamily
\expandafter\def\expandafter\ttfamily\expandafter{\ttfamily
         \not@math@alphabet\tzfamily\mathtz
         \hfontfamily\tzdefault\ks@break}
\let\tzfamily\ttfamily

%% 편의상 다음과 같은 가족바꿈모듬명령도 제공된다. (그래픽, 궁서,
%% 필기, 외곽, 새명조, 목각, 옛글, 봄글씨 및 펜글씨)  이 모듬 명령들은
%% 없어질 잡동사니에 속하므로 되도록 쓰지 않도록 한다.
\DeclareRobustCommand\grfamily{\hfontfamily{gr}}
%\DeclareRobustCommand\gsfamily{\hfontfamily{gs}}
%\DeclareRobustCommand\pgfamily{\hfontfamily{pg}}
%\DeclareRobustCommand\mgfamily{\hfontfamily{mg}}
%\DeclareRobustCommand\ytfamily{\hfontfamily{yt}}
%\DeclareRobustCommand\bmfamily{\hfontfamily{bm}}
%\DeclareRobustCommand\pnfamily{\hfontfamily{pn}}
%\let\smfamily\mjfamily
%\let\olfamily\mjfamily
\DeclareTextFontCommand{\textgr}{\grfamily}
%\DeclareTextFontCommand{\textgs}{\gsfamily}
%\DeclareTextFontCommand{\textpg}{\pgfamily}
%\DeclareTextFontCommand{\textmg}{\mgfamily}
%\DeclareTextFontCommand{\textyt}{\ytfamily}
%\DeclareTextFontCommand{\textbm}{\bmfamily}
%\DeclareTextFontCommand{\textpn}{\pnfamily}
%\let\textsm\textmj
%\let\textol\textmj

%% LaTeX209식의 글자체 바꿈 모듬 명령은 기본 글자체에 해당하는 명령만
%% 제공한다.
\DeclareOldFontCommand{\mj}{\normalhfont\mjfamily}{\@nomath\mj}
\DeclareOldFontCommand{\gt}{\normalhfont\gtfamily}{\@nomath\gt}
\DeclareOldFontCommand{\tz}{\normalhfont\tzfamily}{\@nomath\tz}

%% 우리말의 글자체 초기화는 부호화와 가족만을 초기값으로 바꾼다.
\DeclareRobustCommand\normalhfont
                 {\hfontencoding\hencodingdefault%
                  \hfontfamily\hfamilydefault%
                  \kscfamily\symboldefault\hanguldefault\hanjadefault}

%% \normalfont는 영문과 함께 우리말도 초기화시킨다.
\expandafter\def\expandafter\normalfont\expandafter
  {\normalfont\protect\normalhfont}
\let\reset@font\normalfont

%% 영문 모듬 \usefont는 부호화가 우리말일 경우, 우리말을 다루도록 한다.
\def\usefont#1#2#3#4{\if\hf@encoding#1%
    \hfontencoding{#1}\hfontfamily{#2}\else
    \fontencoding{#1}\fontfamily{#2}\fi\fontseries{#3}%
    \fontshape{#4}\selectfont\ignorespaces}

%% 우리말의 가족계획:
%% ------------------
%% ⑴ 우리말의 인코딩:
%%    우리말은 영문과 다르게, 두 바이트로 한글자를 부호화하므로 영문의
%%    부호화와 구별되도록 다른 부호화를 쓰며, 다음의 모듬으로
%%    지정한다.  부호화의 변경은 새로운 .fd 파일을 요구하게 된다.
\DeclareRobustCommand\hfontencoding[1]{%
    \expandafter\ifx\csname T@#1\endcsname\relax
      \@latex@error{Encoding scheme `#1' unknown}\@eha
    \else
      \edef\hf@encoding{#1}%
      \ifx\cf@encoding\hf@encoding
        \let\enc@update\relax
      \else
        \let\enc@update\@@enc@update
      \fi
    \fi
}

%% ⑵ 우리말글자체의 가족:
%%    우리말가족은 둘로 나뉜다. 앞부분은 심벌/한글/한자의 구성형태를
%%    의미한다.
\DeclareRobustCommand\kscfamily[3]{\edef\sb@{#1}\edef\hg@{#2}\edef\hj@{#3}}

%% 뒷부분은 우리말글자체의 모양새를 의미한다. 명조, 고딕, 타자 및 추가
%% 글자체등의 모양새는 \MapHangulFamily에 의해 각각 한글/심벌/한자의
%% 외부글자체와 연관되어 있다.
\DeclareRobustCommand\hfontfamily[1]{%
  \expandafter\ifx\csname #1@map\endcsname\relax
    \@font@warning{Hangul Fontmap for `#1' undefined\MessageBreak
                   using default map `\expandafter\csname\default@hfamily
                   @map\endcsname' instead\@wrong@font@char}%
    \expandafter\xdef\csname #1@map\endcsname{%
      \expandafter\csname\default@hfamily @map\endcsname}%
    \gdef\default@fontmap{%
      \@font@warning{Some hangul fontmaps were not defined,\MessageBreak
                     default fontmap substituted.\@gobbletwo}}\fi
  \edef\reserved@a{\csname #1@map\endcsname}%
  \expandafter\hfont@map\reserved@a\@nil\ignorespaces}
\def\hfont@map#1,#2,#3\@nil{%
  \edef\hg@family{#1}%
  \edef\sb@family{#2}%
  \edef\hj@family{#3}}
\AtEndDocument{\default@fontmap}
\let\default@fontmap\relax

%% ⑶ 우리말 글자체 시리즈:
%%    우리말글자체시리즈는 영문의 그것과 같다. 다만 \fontseries가 S로
%%    시작할 때 우리말글꼴은 \mdseries를 세번 연속인쇄하여
%%    \bfseries의 效果를 나타나게 한다.
\DeclareRobustCommand\fontseries[1]{%
  \if S\expandafter\@car#1\@nil\@makeboldtrue
    \edef\hf@series{\mddefault}\edef\f@series{\expandafter\@cdr#1\@nil}%
  \else\@makeboldfalse\edef\hf@series{#1}\edef\f@series{#1}\fi}

%% \TeX{}에서 \bfseries의 애초값은 bx이다.  uhc 글자체는 b와 bx가 서로
%% 구분되므로 모듬 명령 \hfontseries에 의해 두꺼운 글자체가 선택되도록
%% 한다.
\DeclareRobustCommand\hfontseries[1]{\edef\hf@series{#1}}

\expandafter\def\expandafter\bfseries\expandafter{\bfseries\hfontseries\hbfdefault}

%% ⑷,⑸ 우리말 글자체모양 및 크기:
%%       우리말의 글자체모양과 크기는 영문의 그것과 동일하게 처리된다.

%% 외부 글자체 파일찾기:
%% ---------------------
%% 우리말글자체는 한 세트가 여러 파일로 나뉘어져 있다. 그러므로
%% 우리말글자체의 외부파일은 다음과 같은 일률적인 규칙에 의거하여
%% 명명한다.
%%  1. 상징기호는 끝숫자가 4, 5, 6, 7로 끝나도록 순서대로 256개씩 나눈다.
%%  2. 한글은 끝숫자가 0부터 9가 되도록 순서대로 256개씩 나눈다.
%%  3. 한자는 끝숫자가 10에서 29가 되도록 순서대로 256개씩 나눈다.
\def\DeclareFontShape@#1#2#3#4#5#6{%
   \expandafter\ifx\csname #1+#2\endcsname\relax
     \@latex@error{Font family `#1+#2' unknown}\@eha
   \else
     \if#1\hf@encoding
       \if\sb@\expandafter\@car#2\@nil\@tempcnta0\def\reserved@b{A,B,C,D}%
       \else\if\hj@\expandafter\@car#2\@nil\@tempcnta2
         \def\reserved@b{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T}%
       \else\@tempcnta1\def\reserved@b{A,B,C,D,E,F,G,H,I,J}\fi\fi
       \@for\@idx:=\reserved@b\do{%
         \expandafter\expandafter\expandafter\@tempcntb\expandafter`\@idx
         \advance\@tempcntb-65
         \ifcase\@tempcnta\def\reserved@c{0}\advance\@tempcntb4%
         \or\def\reserved@c{}%
         \or\def\reserved@c{}\advance\@tempcntb10\fi
         \edef\reserved@c{\reserved@c\number\@tempcntb}%
         \expandafter\xdef\csname#1/#2/#3/#4/\@idx\endcsname{%
           \expandafter\noexpand\csname #5\reserved@c\endcsname}%
         \global\expandafter\let\csname #5\reserved@c\expandafter\endcsname
           \ifx\reserved@a\@empty\@empty\else\reserved@a\fi}%
     \else
       \expandafter\xdef\csname#1/#2/#3/#4\endcsname{%
         \expandafter\noexpand\csname #5\endcsname}%
       \def\reserved@a{#6}%
       \global\expandafter\let\csname#5\expandafter\endcsname
          \ifx\reserved@a\@empty\@empty\else\reserved@a\fi
   \fi\fi
  }
\DeclareSizeFunction{hsub}{\subh@sfcnt\@font@warning}
\DeclareSizeFunction{hssub}{\subh@sfcnt\@font@info}
\def\subh@sfcnt#1{%
    \edef\mandatory@arg{\f@encoding/\mandatory@arg}%
    \begingroup
     \expandafter\split@hname\mandatory@arg/\@nil
     \xdef\reserved@a{\curr@fontshape}%
     \try@load@fontshape
    \endgroup
    \let\f@user@size\f@size
    \expandafter
    \ifx\csname\mandatory@arg\endcsname\relax
      \expandafter\ifx\csname\curr@fontshape!\endcsname\relax
        \errmessage{No\space declaration\space for\space
                  shape\space \mandatory@arg}%
      \global\expandafter\let\csname\curr@fontshape!\endcsname\@empty\fi
      \edef\reserved@b{\expandafter\@car\f@family\@nil}%
      \error@hfontshape
      \edef\reserved@c{\expandafter\csname\f@family @map\endcsname}%
      \expandafter\hfont@map\reserved@c\@nil
      \ifx\sb@\reserved@b\edef\f@family{\sb@\sb@family}\else%
      \ifx\hj@\reserved@b\edef\f@family{\hj@\hj@family}\else%
        \edef\f@family{\hg@\hg@family}\fi\fi
    \else
      \expandafter\ifx\csname\curr@fontshape!\endcsname\relax
        #1{Font\space shape\space `\curr@fontshape'\space in\space
         size\space <\f@size>\space not\space available\MessageBreak
         Font\space shape\space `\reserved@a'\space tried\space
         instead}%
      \global\expandafter\let\csname\curr@fontshape!\endcsname\@empty\fi
      \expandafter\split@hname\mandatory@arg/\@nil
    \fi
    \edef\f@size{\f@user@size}%
    \get@external@hfont
    \do@subst@correction
}
\def\DeclareHFontShape{\begingroup
   \nfss@catcodes
   \expandafter\endgroup
   \DeclareHFontShape@}
\def\DeclareHFontShape@#1#2#3#4#5#6{%
   \expandafter\ifx\csname #1+#2\endcsname\relax
     \@latex@error{Font family `#1+#2' unknown}\@eha
   \else
     \def\reserved@a{#6}%
     \if\sb@\expandafter\@car#2\@nil\def\reserved@b{A,B,C,D}%
     \else\if\hj@\expandafter\@car#2\@nil
       \def\reserved@b{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T}%
     \else\def\reserved@b{A,B,C,D,E,F,G,H,I,J}\fi\fi
     \@for\@idx:=\reserved@b\do{%
       \expandafter\xdef\csname#1/#2/#3/#4/\@idx\endcsname{%
         \expandafter\noexpand\csname #5/\@idx\endcsname}%
       \global\expandafter\let\csname #5/\@idx\expandafter\endcsname
         \ifx\reserved@a\@empty\@empty\else\reserved@a\fi}%
   \fi
  }

%% 우리말 글자체 선택 방법 (HFSS):
%% -------------------------------
%% 우리말은 encoding과 family를 영문과 달리 취급하고 series와 shape,
%% 그리고 size는 영문과 동일하게 취급한다.
%% 우리말의 한가지 글자체는 256개의 글자들로 구성된 여러 글자체로
%% 분리되어 있음으로 지수를 하나 더 추가하여 (심벌: A-D, 한글: A-J,
%% 한자: A-T) 이를 표시한다.(\f@idx)
%% 글자체가 없어서 대치될 때는, 그 글자체의 지수가 없이 그 글자체
%% 세트가 대치되었음을 사용자에게 알리고, 한 글자체 세트마다 한번만
%% 이러한 사실이 알려지도록 한다.  그 대치에는 심벌/한글/한자의
%% \hfamilydefault로 선정된 글자체를 쓴다.  한글의 경우에는
%% 완성|조합/자모를 각각 구분하여 처리한다.
\def\extract@hfont{%
   \get@external@hfont
   \global\expandafter\font\font@name\external@font\relax
    \font@name \relax
    \csname \f@encoding+\f@family\endcsname
    \csname\curr@fontshape\endcsname
    \relax
       }
\def\get@external@hfont{%
   \let\external@font\@empty
   \edef\font@info{\expandafter\expandafter\expandafter\string
        \csname \curr@fontshape/\f@idx \endcsname}%
   \try@size@range
   \ifx\external@font\@empty
      \try@size@substitution
      \ifx\external@font\@empty
         \@latex@error{Font \expandafter \string\font@name\space
                     not found}\@eha
         \edef\reserved@b{\expandafter\@car\f@family\@nil}
         \error@hfontshape
         \edef\reserved@c{\expandafter\csname\f@family @map\endcsname}%
         \expandafter\hfont@map\reserved@c\@nil
         \ifx\sb@\reserved@b\edef\f@family{\sb@\sb@family}\else%
         \ifx\hj@\reserved@b\edef\f@family{\hj@\hj@family}\else%
           \edef\f@family{\hg@\hg@family}\fi\fi
         \get@external@hfont
   \fi\fi
}
\DeclareRobustCommand\selecthfont
        {%
    \ifx\f@linespread\baselinestretch \else
      \set@fontsize\baselinestretch\f@size\f@baselineskip \fi
    \xdef\font@name{%
      \csname\curr@fontshape/\f@idx/\f@size\endcsname}%
    \pickup@hfont
    \font@name
    \size@update
    \enc@update
    \set@hangulskip
    }
\def\pickup@hfont{%
    \expandafter \ifx \font@name \relax
       \define@newhfont
    \fi}
\def\define@newhfont{%
  \begingroup
    \let\typeout\@font@info
    \escapechar\m@ne
    \expandafter\expandafter\expandafter
       \split@hname\expandafter\string\font@name\@nil
      \try@load@fontshape % try always
    \expandafter\ifx
       \csname\curr@fontshape/\f@idx\endcsname \relax
      \wrong@hfontshape\else
      \extract@hfont\fi
  \endgroup}
{\catcode`\/=12
\gdef\split@hname#1/#2/#3/#4/#5/#6\@nil{\def\f@encoding{#1}%
                                        \def\f@family{#2}%
                                        \def\f@series{#3}%
                                        \def\f@shape{#4}%
                                        \def\f@size{#6}}}
\def\DeclareErrorHFont#1#2#3#4#5{%
      \xdef\error@hfontshape{%
          \noexpand\expandafter\noexpand\split@name\noexpand\string
          \expandafter\noexpand\csname#1/#2/#3/#4/#5\endcsname
          \noexpand\@nil}%
      \gdef\default@hfamily{#2}%
      \gdef\default@hseries{#3}%
      \gdef\default@shape{#4}%
      \begingroup
        \edef\reserved@a{\expandafter\csname\default@hfamily @map\endcsname}%
        \expandafter\hfont@map\reserved@a\@nil
        \xdef\sb@family{\sb@family}%
        \xdef\hg@family{\hg@family}%
        \xdef\hj@family{\hj@family}%
      \endgroup
      \global\let\hf@series\default@hseries
      \global\let\f@shape\default@shape
      \gdef\f@size{#5}%
      \gdef\f@baselineskip{#5pt}%
}
\@onlypreamble\DeclareErrorHFont
\def\wrong@hfontshape{%
    \csname D@\f@encoding\endcsname      % install defaults if in math
    \edef\reserved@a{\csname\curr@fontshape/\f@idx\endcsname}%
    \edef\reserved@b{\expandafter\string\csname\curr@fontshape\endcsname}%
  \ifx\last@fontshape\reserved@a
     \errmessage{Corrupted NFSS tables}%
     \edef\reserved@c{\expandafter\@car\f@family\@nil}%
     \error@hfontshape
     \edef\reserved@d{\expandafter\csname\f@family @map\endcsname}%
     \expandafter\hfont@map\reserved@d\@nil
     \ifx\sb@\reserved@c\edef\f@family{\sb@\sb@family}\else%
     \ifx\hj@\reserved@c\edef\f@family{\hj@\hj@family}\else%
       \edef\f@family{\hg@\hg@family}\fi\fi
  \else
    \let\f@shape\default@shape
    \expandafter\ifx\csname\curr@fontshape/\f@idx\endcsname\relax
        \let\f@series\default@hseries
        \expandafter
        \ifx\csname\curr@fontshape/\f@idx\endcsname\relax
          \edef\reserved@d{\expandafter\csname\default@hfamily @map\endcsname}%
          \expandafter\hfont@map\reserved@d\@nil
          \if\sb@\expandafter\@car\f@family\@nil
              \edef\f@family{\sb@\sb@family}\else
          \if\hj@\expandafter\@car\f@family\@nil
              \edef\f@family{\hj@\hj@family}\else
              \edef\f@family{\hg@\hg@family}\fi\fi
        \fi \fi
  \fi
    \expandafter\ifx\csname\reserved@b!\endcsname\relax
       \@font@warning{Font shape `\expandafter\string\reserved@b'
                       \expandafter\@gobble\string\@undefined\MessageBreak
                     using `\curr@fontshape' instead\@wrong@font@char}%
      \global\expandafter\let\csname\reserved@b!\endcsname\@empty\fi
    \global\let\last@fontshape\reserved@a
    \gdef\@defaultsubs{%
      \@font@warning{Some font shapes were not available, defaults
                      substituted.\@gobbletwo}}%
    \global\expandafter\expandafter\expandafter\let
       \expandafter\reserved@a
           \csname\curr@fontshape/\f@idx\endcsname
    \xdef\font@name{%
      \csname\curr@fontshape/\f@idx/\f@size\endcsname}%
    \pickup@hfont}
\def\DeclareHFontEncoding{%
   \begingroup
   \nfss@catcodes
   \expandafter\endgroup
   \DeclareHFontEncoding@}
\@onlypreamble\DeclareHFontEncoding
\def\DeclareHFontEncoding@#1#2#3{%
  \expandafter
  \ifx\csname T@#1\endcsname\relax
     \def\cdp@elt{\noexpand\cdp@elt}%
     \begingroup
     \edef\reserved@a{\csname\default@hfamily @map\endcsname}
     \expandafter\hfont@map\reserved@a\@nil
     \xdef\cdp@list{\cdp@list%
                    \cdp@elt{#1}{\symboldefault\sb@family}%
                    {\default@hseries}{\default@shape}%
                    \cdp@elt{#1}{\hanguldefault\hg@family}%
                    {\default@hseries}{\default@shape}%
                    \cdp@elt{#1}{\hanjadefault\hj@family}%
                    {\default@hseries}{\default@shape}}%
     \endgroup
     \expandafter\let\csname#1-cmd\endcsname\@changed@cmd
  \else
     \@font@info{Redeclaring font encoding #1}%
  \fi
  \global\@namedef{T@#1}{#2}%
  \global\@namedef{M@#1}{\default@M#3}%
  }
\@onlypreamble\DeclareHFontEncoding@
\def\DeclareHFontSubstitution#1#2#3#4{%
  \expandafter
  \ifx\csname T@#1\endcsname\relax
    \@latex@error{Encoding scheme  `#1' unknown}\@eha
  \else
    \begingroup
       \edef\reserved@a{\csname#2@map\endcsname}
       \expandafter\hfont@map\reserved@a\@nil
       \def\reserved@a{#1}%
       \toks@{}%
       \let\reserved@d\@empty
       \def\cdp@elt##1##2##3##4{%
          \def\reserved@b{##1}%
          \ifx\reserved@a\reserved@b
            \ifx\reserved@d\@empty
              \edef\reserved@c{\noexpand\cdp@elt{#1}{\sb@\sb@family}{#3}{#4}%
                               \noexpand\cdp@elt{#1}{\hg@\hg@family}{#3}{#4}%
                               \noexpand\cdp@elt{#1}{\hj@\hj@family}{#3}{#4}}%
              \let\reserved@d\relax
              \expandafter\addto@hook
              \expandafter\toks@\expandafter{\reserved@c}\fi%
          \else
             \addto@hook\toks@{\cdp@elt{##1}{##2}{##3}{##4}}%
          \fi}%
        \cdp@list
        \xdef\cdp@list{\the\toks@}%
    \endgroup
    \global\@namedef{D@#1}{%
        \def\default@hfamily{#2}%
        \def\default@hseries{#3}%
        \def\default@shape{#4}%
        }%
  \fi
 }
\@onlypreamble\DeclareHFontSubstitution

%% HFSS의 설정 확인:
%% -----------------
%% 우리말의 한 가족은 심벌/한글/한자의 세가지 외부 글자체와 연관되어
%% 있다. 우리말 문서가 시작하기 전에, 기본값으로 설정된
%% 심벌/한글/한자의 대치 글자체와 착오시 사용될 글자체가 제대로
%% 설정되어 있는지 확인함으로서 글자체 선택시 발생할 수 재앙을 미리
%% 방지한다.
\def\process@table{%
    \def\cdp@elt##1##2##3##4{%
        \@font@info{Checking defaults for
                  ##1/##2/##3/##4}%
      \if\hf@encoding##1
        \expandafter
        \ifx\csname##1/##2/##3/##4/A\endcsname\relax
          \begingroup
           \def\f@encoding{##1}\def\f@family{##2}%
           \try@load@fontshape
          \endgroup
        \fi
        \expandafter
        \ifx\csname##1/##2/##3/##4/A\endcsname\relax
             \@latex@error{This HFSS system isn't set up properly}%
                       {For hangul encoding scheme ##1 the defaults
                        ##2/##3/##4 do not form a valid font shape}%
        \else
             \@font@info{... okay}%
        \fi
      \else
        \expandafter
        \ifx\csname##1/##2/##3/##4\endcsname\relax
          \begingroup
           \def\f@encoding{##1}\def\f@family{##2}%
           \try@load@fontshape
          \endgroup
        \fi
        \expandafter
        \ifx\csname##1/##2/##3/##4\endcsname\relax
             \@latex@error{This NFSS system isn't set up properly}%
                       {For encoding scheme ##1 the defaults
                        ##2/##3/##4 do not form a valid font shape}%
        \else
             \@font@info{... okay}%
        \fi
      \fi}%
    \cdp@list
    \begingroup
       \escapechar\m@ne
       \error@fontshape
       \expandafter\ifx\csname \curr@fontshape\endcsname\relax
          \begingroup
            \try@load@fontshape
           \endgroup
       \fi
       \expandafter\ifx\csname \curr@fontshape\endcsname\relax
         \@latex@error{This NFSS system isn't set up properly}%
            {The system maintainer forgot to specify a suitable
             substitution
             font shape using the \noexpand\DeclareErrorFont
             command}%
       \fi
       \expandafter\ifx\csname\hfamilydefault @map\endcsname\relax
         \@latex@error{This HFSS system isn't set up properly}%
            {The system maintainer forgot to specify a suitable
             fontmap for default hangul family `\hfamilydefault'
             using the \noexpand\MapHangulFamily command}%
       \fi
       \error@hfontshape
       \edef\reserved@a{\expandafter\csname\f@family @map\endcsname}%
       \expandafter\hfont@map\reserved@a\@nil
       \edef\f@family{\sb@\sb@family}%
       \expandafter\ifx\csname \curr@fontshape/A\endcsname\relax
          \begingroup
            \try@load@fontshape
           \endgroup
       \fi
       \expandafter\ifx\csname \curr@fontshape/A\endcsname\relax
         \@latex@error{This HFSS system isn't set up properly}%
            {The system maintainer forgot to specify a suitable
             substitution symbol
             font shape using the \noexpand\DeclareErrorHFont
             command or \noexpand\MapHangulFamily command}%
       \fi
       \edef\f@family{\hg@\hg@family}%
       \expandafter\ifx\csname \curr@fontshape/A\endcsname\relax
          \begingroup
            \try@load@fontshape
           \endgroup
       \fi
       \expandafter\ifx\csname \curr@fontshape/A\endcsname\relax
         \@latex@error{This HFSS system isn't set up properly}%
            {The system maintainer forgot to specify a suitable
             substitution hangul
             font shape using the \noexpand\DeclareErrorHFont
             command or \noexpand\MapHangulFamily command}%
       \fi
       \edef\f@family{\hj@\hj@family}%
       \expandafter\ifx\csname \curr@fontshape/A\endcsname\relax
          \begingroup
            \try@load@fontshape
           \endgroup
       \fi
       \expandafter\ifx\csname \curr@fontshape/A\endcsname\relax
         \@latex@error{This HFSS system isn't set up properly}%
            {The system maintainer forgot to specify a suitable
             substitution hanja
             font shape using the \noexpand\DeclareErrorHFont
             command or \noexpand\MapHangulFamily command}%
       \fi
    \endgroup
    \let\select@group\document@select@group
    \hfontencoding{\hencodingdefault}%
    \hfontfamily{\hfamilydefault}%
    \fontencoding{\encodingdefault}%
    \fontfamily{\familydefault}%
    \fontseries{\seriesdefault}%
    \fontshape{\shapedefault}%
 \everyjob{}%
}

%% 우리말 글자체의 기본값:
%% -----------------------
%% 아무것도 지정하지 않으면 완성형 명조체가 된다.
\newcommand\hencodingdefault{H}

\newcommand\symboldefault{s}
\newcommand\hanguldefault{w}
\newcommand\hanjadefault{h}
\newcommand\mjdefault{mj}
\newcommand\gtdefault{gt}
\newcommand\tzdefault{tz}
\newcommand\hfamilydefault{\mjdefault}
\if@makebold\newcommand\hbfdefault{m}
\else\newcommand\hbfdefault{b}\fi

%% 우리말가족 이름에 따른 외부 글자체의 설정
%% -----------------------------------------
%%      \MapHangulFamily{우리말가족}{한글글자체,심벌글자체,한자글자체}
%%                      (글자체이름 = 한글/심벌/한자글꼴)
\DeclareRobustCommand\MapHangulFamily[2]{%
  \expandafter\edef\csname #1@map\endcsname{#2}}

%% 기본글자체
\MapHangulFamily{mj}{wmj,wmj,wmj}
\MapHangulFamily{gt}{wgt,wgt,wgt}
\MapHangulFamily{tz}{wtt,wtt,wtt}
\MapHangulFamily{gr}{wgr,wgr,wgt}

%% 추가글자체
\InputIfFileExists{koextrafonte.tex}{}{}

%% \DeclareErrorHFont{H}{\mjdefault}{m}{n}{10}
%% \DeclareHFontSubstitution{H}{\mjdefault}{m}{n}

%% hfont.cfg에서 이들을 미리 지정/수정할 수 있다.
\InputIfFileExists{hfont.cfg}{}{}

\kscfamily{\symboldefault}{\hanguldefault}{\hanjadefault}

\DeclareErrorHFont{H}{\mjdefault}{m}{n}{10}
\DeclareHFontEncoding{\hencodingdefault}{}{}
\DeclareHFontSubstitution{H}{\mjdefault}{m}{n}
\hfontencoding\hencodingdefault

%% 우리말 찾기:
%% ------------
%% 우리말은 모두 \catcode=13으로 처리되며 우리말 부호 영역의
%% 두 바이트가 한 글자를 형성한다. 이 두 개의 바이트를 분석하여
%% 외부 글꼴의 지수와 심벌/한글/한자 중 하나를 확정한다.
%%
\begingroup
\catcode`^^98\active
\catcode`^^99\active
\catcode`^^a0\active
\def^^98#1#2#3{\xdef#1##1{\noexpand\h@C{\hf@}{\noexpand\ifnum`##1<#2
    D\noexpand\else\noexpand\ifnum`##1>#3 C\noexpand\else
    A\noexpand\fi\noexpand\fi}{\noexpand#1}{##1}}} 
\def^^99#1#2{\xdef#1##1{\noexpand\h@C{\hf@}{#2}{\noexpand#1}{##1}}}
\def^^a0#1#2#3/#4{\xdef#1##1{\noexpand\h@C{\hf@}{\noexpand\ifnum`##1<#2
    #3\noexpand\else#4\noexpand\fi}{\noexpand#1}{##1}}}

%% 심벌
\def\hf@{sb}
%^^99^^a1B
% 금칙 문자: ’”〕〉》」』】의 앞과
%           ‘“〔〈《《『【 위 뒤    (2005/04/09 koaunghi@kornet.net)
\gdef\^^96#1{\ifx#1^^af\spacefactor=999
  \else\ifx#1^^b1\spacefactor=999
  \else\ifx#1^^b3\spacefactor=999
  \else\ifx#1^^b5\spacefactor=999
  \else\ifx#1^^b7\spacefactor=999
  \else\ifx#1^^b9\spacefactor=999
  \else\ifx#1^^bb\spacefactor=999
  \else\ifx#1^^bd\spacefactor=999
  \fi\fi\fi\fi\fi\fi\fi\fi}
\gdef\^^97#1{\ifx#1^^ae\spacefactor=999
  \else\ifx#1^^b0\spacefactor=999
  \else\ifx#1^^b2\spacefactor=999
  \else\ifx#1^^b4\spacefactor=999
  \else\ifx#1^^b6\spacefactor=999
  \else\ifx#1^^b8\spacefactor=999
  \else\ifx#1^^ba\spacefactor=999
  \else\ifx#1^^bc\spacefactor=999
  \fi\fi\fi\fi\fi\fi\fi\fi}
\xdef^^a1#1{\noexpand\^^96{#1}\noexpand\h@C{\hf@}{B}{\noexpand^^a1}{#1}\noexpand\^^97{#1}}
^^99^^a2B
\xdef^^a3#1{\noexpand\h@C{\hf@}{\noexpand\ifnum\expandafter`\noexpand#1="0DC
    A\noexpand\else D\noexpand\fi}{\noexpand^^a3}{\noexpand#1}}%
^^99^^a4A^^99^^a5D^^99^^a6C^^99^^a7B^^98^^a8{"0B0}{"0F5}
^^98^^a9{"0B1}{"0F5}^^99^^aaC^^99^^abC^^99^^acD

%%% 한글
\def\hf@{hg}
^^99^^b0A^^99^^b1A^^a0^^b2{"0E5}A/B^^99^^b3B^^99^^b4B^^a0^^b5{"0CB}B/C
^^99^^b6C^^99^^b7C^^a0^^b8{"0B1}C/D^^99^^b9D^^a0^^ba{"0F5}D/E^^99^^bbE
^^99^^bcE^^a0^^bd{"0DB}E/F^^99^^beF^^99^^bfF^^a0^^c0{"0C1}F/G^^99^^c1G
^^99^^c2G^^a0^^c3{"0A7}G/H^^99^^c4H^^a0^^c5{"0EB}H/I^^99^^c6I^^99^^c7I
^^a0^^c8{"0D1}I/J

%%% 漢字
\def\hf@{hj}
^^99^^caA^^99^^cbA^^a0^^cc{"0E5}A/B^^99^^cdB^^99^^ceB^^a0^^cf{"0CB}B/C
^^99^^d0C^^99^^d1C^^a0^^d2{"0B1}C/D^^99^^d3D^^a0^^d4{"0F5}D/E^^99^^d5E
^^99^^d6E^^a0^^d7{"0DB}E/F^^99^^d8F^^99^^d9F^^a0^^da{"0C1}F/G^^99^^dbG
^^99^^dcG^^a0^^dd{"0A7}G/H^^99^^deH^^a0^^df{"0EB}H/I^^99^^e0I^^99^^e1I
^^a0^^e2{"0D1}I/J^^99^^e3J^^99^^e4J^^a0^^e5{"0B7}J/K^^99^^e6K
^^a0^^e7{"0FB}K/L^^99^^e8L^^99^^e9L^^a0^^ea{"0E1}L/M^^99^^ebM^^99^^ecM
^^a0^^ed{"0C7}M/N^^99^^eeN^^99^^efN^^a0^^f0{"0AD}N/O^^99^^f1O
^^a0^^f2{"0F1}O/P^^99^^f3P^^99^^f4P^^a0^^f5{"0D7}P/Q^^99^^f6Q^^99^^f7Q
^^a0^^f8{"0BD}Q/R^^99^^f9R^^99^^faR^^a0^^fb{"0A3}R/S^^99^^fcS
^^a0^^fd{"0E7}S/T
\endgroup

%% 이해할 수 없는 오류: Undefined control sequence with ^^c9
\let^^c9\relax

%% 우리말을 최종 처리할 때는, 흩어져 있는 우리말 글자체 정보를
%% 수집하여 해당하는 외부 글자체를 찾은 후 인쇄한다. softbold가
%% 요구되면 두 번 더 중첩 인쇄하도록 한다.
\let\KSC@\string
\let\f@idx\relax
\def\h@C#1#2#3#4{%
  \ifx\protect\@typeset@protect\begingroup
    \edef\f@encoding{\hf@encoding}%
    \edef\f@family{\csname #1@\endcsname\csname #1@family\endcsname}%
    \edef\f@series{\hf@series}\gdef\f@idx{#2}%
    \selecthfont\@Hyphen\hemph@size{\KSC@#3\KSC@#4\if@makebold
      \hbox to0.03ex{\hss\KSC@#3\KSC@#4}%
      \hbox to0.03ex{\hss\KSC@#3\KSC@#4}\fi}\endgroup
  \else\KSC@#3\KSC@#4\fi}

\def\no@ccent#1{#1}
\let\hemph@size\no@ccent

%%%
%%% Kim Dohyun's AUTOJOSA solution.
%%%
%%% hyper@link 재정의
\AtBeginDocument{%
    \@ifpackageloaded{atveryend}{\AtVeryEndDocument{\let\protect\relax}}{}%
    \providecommand\@firstoffive [5]{#1}%
    \providecommand\@secondoffive[5]{#2}%
    \providecommand\@thirdoffive [5]{#3}%
    \providecommand\@fourthoffive[5]{#4}%
    \@ifundefined{hyper@link}%
        {\PackageWarningNoLine{kotex}%
            {hyperref을 로드하여야 자동조사가 작동합니다}}%
        {\let\hyper@link@ORIG\hyper@link
         \def\hyper@link#1#2#3{\hyper@link@ORIG{#1}{#2}{#3}%
           \begingroup\let\null\@empty\xdef\make@josa{#3}\endgroup
         }}%
}

%% `josa.tab`을 불러온다.
%% from hangul.sty
\begingroup
\IfFileExists{josa.tab}{%
  \newread\JS@tab
  \endlinechar\m@ne
  \def\JS@{\read\JS@tab to\@t \expandafter\split@t\@t\relax
    \ifnum\count@=2 \let\next\relax \else
      \ifcase\count@\let\next=2 \or\let\next=1 \fi%%%modified
      \global\expandafter\let\csname\reserved@a\endcsname\next
      \let\next\JS@ \fi \next}
  \def\split@t##1,##2,##3\relax{\count@##1\def\reserved@a{##2|##3}}%
  \openin\JS@tab=josa.tab \JS@ \closein\JS@tab}%
{\PackageWarningNoLine{\string\HLaTeX}{``josa.tab''이 없습니다!!!^^J
 \@spaces\@spaces\@spaces\@spaces\@spaces\@spaces
 인용에 사용되는 자동조사는 잘못 처리될 수 있읍니다.}}
\endgroup
%
%%% 한글, 기호문자, 영문 자동조사 처리. \nameref 땜에 토큰 4개까지 불러옴
\providecommand*{\josa@LastThreeChar}[1]{%
  \@ifemptyarg{#1}{0000}{\expandafter\@lastthreechar#1`\^^M}}
\def\@lastthreechar#1#2`\^^M{%
  \@ifemptyarg{#2}{000#1}{\@@lastthreechar#1#2`\^^M}}
\def\@@lastthreechar#1#2#3`\^^M{%
  \@ifemptyarg{#3}{00#1#2}{\@@@lastthreechar#1#2#3`\^^M}}
\def\@@@lastthreechar#1#2#3#4`\^^M{%
  \@ifemptyarg{#4}{0#1#2#3}{\@@@@lastthreechar#1#2#3#4`\^^M}}
\def\@@@@lastthreechar#1#2#3#4#5`\^^M{%
  \@ifemptyarg{#5}{#1#2#3#4}{\@@@@lastthreechar#2#3#4#5`\^^M}}
\providecommand{\@ifemptyarg}[1]{% {absence}{presence}
  \ifx\@empty#1\@empty
   \expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi}
\def\@josa#1#2{%
  \def\@jung{#1}\def\@jong{#2}\def\ri@ul{\@ifemptyarg{#1}{}{#2}}%
  \edef\lastthree@make@josa{\josa@LastThreeChar{\make@josa}}%
  \edef\@zeroth{\expandafter\@firstoffive\lastthree@make@josa\@empty}%
  \edef\@first{\expandafter\@secondoffive\lastthree@make@josa\@empty}%
  \edef\@second{\expandafter\@thirdoffive\lastthree@make@josa\@empty}%
  \edef\@third{\expandafter\@fourthoffive\lastthree@make@josa\@empty}%
  \expandafter\ifx\@third\relax %%% \nameref는 \relax를 달고 있다
    \let\@third\@second
    \let\@second\@first
    \let\@first\@zeroth
  \fi
  \expandafter\ifx\@third\endgroup
%% 한글/기호문자 처리루틴.
    \count@\expandafter`\@first
    \@tempcnta\count@ \divide\@tempcnta\sixt@@n
    \@tempcntb\@tempcnta \multiply\@tempcntb\sixt@@n
    \advance\count@-\@tempcntb
    \edef\reserved@a{\hexnumber@{\@tempcnta}\hexnumber@{\count@}}%
    \count@\expandafter`\@second
    \@tempcnta\count@ \divide\@tempcnta\sixt@@n
    \@tempcntb\@tempcnta \multiply\@tempcntb\sixt@@n
    \advance\count@-\@tempcntb
    \edef\reserved@b{\hexnumber@{\@tempcnta}\hexnumber@{\count@}}%
    \expandafter\if\csname\reserved@a|\reserved@b\endcsname 1\ri@ul
      \else\expandafter\if\csname\reserved@a|\reserved@b\endcsname 2\@jung
      \else\@jong\fi\fi
%% 아래는 영문숫자 처리루틴.
  \else
    \let\@last\@third
    \if n\@second\if g\@third\let\@last=0\fi\fi%skating
    \if a\@second\if p\@third\let\@last=0\fi\fi%cap
    \if u\@second\if p\@third\let\@last=0\fi\fi%cup
    \if a\@second\if t\@third\let\@last=0\fi\fi%cat
    \if e\@second\if t\@third\let\@last=0\fi\fi%Hamlet
    \if i\@second\if t\@third\let\@last=0\fi\fi%summit
    \if o\@second\if t\@third\let\@last=0\fi\fi%not
    \if u\@second\if t\@third\let\@last=0\fi\fi%nut
    \if o\@second\if k\@third\let\@last=0\fi\fi%book
    \if i\@second\if c\@third\let\@last=0\fi\fi%picnic
    \if l\@second\if e\@third\let\@last=1\fi\fi%apple
    \if i\@first\if m\@second\if e\@third\let\@last=0\fi\fi\fi%time
    \if i\@first\if n\@second\if e\@third\let\@last=0\fi\fi\fi%mine
    \if a\@first\if c\@second\if k\@third\let\@last=0\fi\fi\fi%back
    \if i\@first\if c\@second\if k\@third\let\@last=0\fi\fi\fi%pick
    \if o\@first\if a\@second\if t\@third\let\@last=2\fi\fi\fi%boat
    \if T\@first\if e\@second\if X\@third\let\@last=0\fi\fi\fi%TeX
    \if 0\@last\@jong\else
      \if 1\@last\ri@ul\else
      \if 2\@last\@jung\else
      \if 3\@last\@jong\else
      \if 4\@last\@jung\else
      \if 5\@last\@jung\else
      \if 6\@last\@jong\else
      \if 7\@last\ri@ul\else
      \if 8\@last\ri@ul\else
      \if 9\@last\@jung\else
      \if l\@last\ri@ul\else
      \if m\@last\@jong\else
      \if n\@last\@jong\else
      \if L\@last\ri@ul\else
      \if M\@last\@jong\else
      \if N\@last\@jong\else
      \@jung
          \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
  \fi
}
\def\make@josa{00}

%%%% From File: ltxref.dtx
\def\@setref#1#2#3{%
  \let\protect\relax
  \ifx#1\relax
   \protect\G@refundefinedtrue
   \nfss@text{\reset@font\bfseries ??}%
   \@latex@warning{Reference `#3' on page \thepage \space
             undefined}%
  \else
   \expandafter#2#1\null
  \fi}
\def\label#1{\@bsphack
  \protected@write\@auxout{}%
         {\string\newlabel{#1}%
          {{\@currentlabel}%
           {\thepage}}}%
  \@esphack}
\def\ref#1{\let\protect\string
        \expandafter\@setref\csname r@#1\endcsname\@firstoftwo{#1}}
\def\pageref#1{\let\protect\string
          \expandafter\@setref\csname r@#1\endcsname\@secondoftwo{#1}}
\def\newlabel{\let\protect\string\@newl@bel r}%

%%%
%%% 자동조사명령 및 글자체바꿈 우리말 명령:
%%%   \은/\는 \이/\가 \을/\를 \와/\과 \으로/\로 (\으로서/\로서 \으로써/\로써)
%%%   \옛글\외곽\명조\목각\고딕\그래픽\궁서\새명조\필기\펜글씨\펜흘림\봄글씨
%%%
%% nojosa-gana
%% This is a part of hangul-nojosa.sty
%%
%\makeatletter
\def\jaso#1{\@jaso{\@nameuse{c@#1}}}
\def\@jaso#1{\ifcase#1\or ㄱ\or ㄴ\or ㄷ\or ㄹ\else\@ijaso{#1}\fi}
\def\@ijaso#1{\ifcase#1\or\or\or\or\or ㅁ\or ㅂ\or ㅅ\or ㅇ\or ㅈ\or
  ㅊ\or ㅋ\or ㅌ\or ㅍ\or ㅎ\else\@ctrerr\fi}
\def\gana#1{\@gana{\@nameuse{c@#1}}}
\def\@gana#1{\ifcase#1\or 가\or 나\or 다\or 라\else\@igana{#1}\fi
  }
\def\@igana#1{\ifcase#1\or\or\or\or\or 마\or 바\or 사\or 아\or 자\or
  차\or 카\or 타\or 파\or 하\else\@ctrerr\fi}
\def\ojaso#1{\@ojaso{\@nameuse{c@#1}}}
\def\@ojaso#1{\ifcase#1\or ㉠\or ㉡\or ㉢\or
  ㉣\else\@iojaso{#1}\fi}
\def\@iojaso#1{\ifcase#1\or\or\or\or\or ㉤\or ㉥\or ㉦\or ㉧\or ㉨\or
  ㉩\or ㉪\or ㉫\or ㉬\or ㉭\else\@ctrerr\fi}
\def\ogana#1{\@ogana{\@nameuse{c@#1}}}
\def\@ogana#1{\ifcase#1\or ㉮\or ㉯\or ㉰\or ㉱\else\@iogana{#1}\fi
  }
\def\@iogana#1{\ifcase#1\or\or\or\or\or ㉲\or ㉳\or ㉴\or ㉵\or ㉶\or
  ㉷\or ㉸\or ㉹\or ㉺\or ㉻\else\@ctrerr\fi}
\def\pjaso#1{\@pjaso{\@nameuse{c@#1}}}
\def\@pjaso#1{\ifcase#1\or ㈀\or ㈁\or ㈂\or
  ㈃\else\@ipjaso{#1}\fi}
\def\@ipjaso#1{\ifcase#1\or\or\or\or\or ㈄\or ㈅\or ㈆\or ㈇\or ㈈\or
  ㈉\or ㈊\or ㈋\or ㈌\or ㈍\else\@ctrerr\fi}
\def\pgana#1{\@pgana{\@nameuse{c@#1}}}
\def\@pgana#1{\ifcase#1\or ㈎\or ㈏\or ㈐\or ㈑\else\@ipgana{#1}\fi
  }
\def\@ipgana#1{\ifcase#1\or\or\or\or\or ㈒\or ㈓\or ㈔\or ㈕\or ㈖\or
  ㈗\or ㈘\or ㈙\or ㈚\or ㈛\else\@ctrerr\fi}
\def\onum#1{\@onum{\@nameuse{c@#1}}}
\def\@onum#1{\ifcase#1\or ①\or ②\or ③\or ④\else\@ionum{#1}\fi
  \ifnum#1<\sixt@@n\fi}
\def\@ionum#1{\ifcase#1\or\or\or\or\or ⑤\or ⑥\or ⑦\or ⑧\or ⑨\or
  ⑩\or ⑪\or ⑫\or ⑬\or ⑭\or ⑮\else\@ctrerr\fi}
\def\pnum#1{\@pnum{\@nameuse{c@#1}}}
\def\@pnum#1{\ifcase#1\or ⑴\or ⑵\or ⑶\or ⑷\else\@ipnum{#1}\fi
  \ifnum#1<\sixt@@n\fi}
\def\@ipnum#1{\ifcase#1\or\or\or\or\or ⑸\or ⑹\or ⑺\or ⑻\or ⑼\or
  ⑽\or ⑾\or ⑿\or ⒀\or ⒁\or ⒂\else\@ctrerr\fi}
\def\oeng#1{\@oeng{\@nameuse{c@#1}}}
\def\@oeng#1{\ifcase#1\or ⓐ\or ⓑ\or ⓒ\or ⓓ\else\@ioeng{#1}\fi
  }
\def\@ioeng#1{\ifcase#1\or\or\or\or\or ⓔ\or ⓕ\or ⓖ\or ⓗ\or ⓘ\or
  ⓙ\or ⓚ\or ⓛ\or ⓜ\or ⓝ\or ⓞ\or ⓟ\or ⓠ\or ⓡ\or ⓢ\or ⓣ\or
  ⓤ\or ⓥ\or ⓦ\or ⓧ\or ⓨ\or ⓩ\else\@ctrerr\fi}
\def\peng#1{\@peng{\@nameuse{c@#1}}}
\def\@peng#1{\ifcase#1\or ⒜\or ⒝\or ⒞\or ⒟\else\@ipeng{#1}\fi
  }
\def\@ipeng#1{\ifcase#1\or\or\or\or\or ⒠\or ⒡\or ⒢\or ⒣\or ⒤\or
  ⒥\or ⒦\or ⒧\or ⒨\or ⒩\or ⒪\or ⒫\or ⒬\or ⒭\or ⒮\or ⒯\or
  ⒰\or ⒱\or ⒲\or ⒳\or ⒴\or ⒵\else\@ctrerr\fi}
\def\hnum#1{\@hnum{\@nameuse{c@#1}}}
%%\def\@hnum#1{\ifcase#1\or 하나\or 둘\or 셋\or 넷\or\@ihnum{#1}\fi} %% removed. hangul-k.
\def\@hnum#1{\ifcase#1\or 하나\or 둘\or 셋\or 넷\or 다섯\or 여섯\or 일곱\or 여덟\or
  아홉\or 열\or 열하나\or 열둘\or 열셋\or 열넷\or 열다섯\or 열여섯\or
  열일곱\or 열여덟\or 열아홉\or 스물\or 스물하나\or 스물둘\or
  스물셋\or 스물넷\else\@ctrerr\fi}
\def\Hnum#1{\@Hnum{\@nameuse{c@#1}}}
\def\@Hnum#1{\ifcase#1\or 첫\or 둘\or 셋\or 넷\or\@iHnum{#1}\fi 째}
%%% 세째, 네째를 셋째, 넷째로 바꿈. -- hangul-k.
\def\@iHnum#1{\ifcase#1\or\or\or\or\or 다섯\or 여섯\or 일곱\or 여덟\or
  아홉\or 열\or 열한\or 열두\or 열셋\or 열넷\or 열다섯\or 열여섯\or
  열일곱\or 열여덟\or 열아홉\or 스무\or 스물한\or 스물두\or 스물셋\or
  스물넷\else\@ctrerr\fi 째} 
%%% hangul-k adds the following two commands.
\def\hroman#1{\@hroman{\@nameuse{c@#1}}}
\def\@hroman#1{\ifcase#1\or ⅰ\or ⅱ\or ⅲ\or
        ⅳ\or ⅴ\or ⅵ\or ⅶ\or ⅷ\or ⅸ\or ⅹ\else\@ctrerr\fi}
\def\hRoman#1{\@hRoman{\@nameuse{c@#1}}}
\def\@hRoman#1{\ifcase#1\or Ⅰ\or Ⅱ\or Ⅲ\or
        Ⅳ\or Ⅴ\or Ⅵ\or Ⅶ\or Ⅷ\or Ⅸ\or Ⅹ\else\@ctrerr\fi}

%%% 자동음운변화 명령. 
%%%
%%% "\이라" 구현을 위한 추가. (DohyunKim) from latex.ltx.
\long\def\@ifnextchar@honorspace#1#2#3{%
  \let\reserved@d=#1%
  \def\reserved@a{#2}%
  \def\reserved@b{#3}%
  \futurelet\@let@token\@ifnch@honorspace}
\def\@ifnch@honorspace{%
%  \ifx\@let@token\@sptoken
%    \let\reserved@c\@xifnch
%  \else
    \ifx\@let@token\reserved@d
      \let\reserved@c\reserved@a
    \else
      \let\reserved@c\reserved@b
    \fi
%  \fi
  \reserved@c}
%% 우리말 조사 명령.
\def\^^c0{%
      \@ifnextchar^^da{\f@urj@mo}%
      {\@ifnextchar^^cc{\f@urIjos@}{\f@urjos@}}%
}
\def\f@urIjos@^^cc{%
      \@ifnextchar@honorspace^^b6{\f@urIRAjos@}{\가}%  이(C0CC)
}
\def\f@urIRAjos@^^b6{%
  \@ifnextchar@honorspace^^f3{\라\@gobble}%		이라(C0CC B6F3)
    {\PackageError{kotex}{이런 명령은 없습니다}{}}%
}
\def\f@urjos@#1{%
%%  \ifx#1^^cc\@josa{가}{이}\else%     이(C0CC)
  \ifx#1^^ba\@josa{는}{은}\else%      은(C0BA)
  \ifx#1^^bb\@josa{를}{을}\else%      을(C0BB)
  \ifx#1^^b8\@josa{}{으}%             으(C0B8) 로(서/써)
  \fi\fi\fi%
}
%
%\def\f@urj@mo^^da모#1#2#3#4{% 자모(C0DAB8F0)
%  \ifx#1^^b8\hfontfamily{jmj}\else% 명조(B8EDC1B6)
%  \ifx#1^^b0\hfontfamily{jgt}\else% 고딕(B0EDB5F1)
%  \ifx#1^^b3\hfontfamily{jnv}\else% 노벨(B3EBBAA7)
%  \ifx#1^^bc\hfontfamily{jsr}%      소라(BCD2B6F3)
%  \fi\fi\fi\fi\ignorespaces}%
\def\는{\은}%   는(B4C2)
\def\로{\@josa{}{으}로}%                        로(B7CE) (서/써)
\def\라{\@josa{라}{이라}}%                      라(B6F3)
\def\와{\@josa{와}{과}}%                        와(BFCD)
%\def\^^bf{%
%  \@ifnextchar^^cd{\@josa{와}{과}\@gobble}\yt@or@ol}% 와(BFCD)
%\def\yt@or@ol#1#2#3{%
%  \ifx#1^^be\hfontfamily{yt}\else%                                      옛글(BFBDB1BD)
%  \ifx#1^^dc\hfontfamily{ol}\fi\fi\ignorespaces}%       외곽(BFDCB0FB)
\def\^^b8{\@ifnextchar^^a6{\을\@gobble}\mj@or@mg}%      를(B8A6)
\def\mj@or@mg#1#2#3{%
  \ifx#1^^ed\hfontfamily{mj}\else%                                      명조(B8EDC1B6)
  \fi\ignorespaces}
%\def\mj@or@mg#1#2#3{%
%  \ifx#1^^ed\hfontfamily{mj}\else%                                      명조(B8EDC1B6)
%  \ifx#1^^f1\hfontfamily{mg}\fi\fi\ignorespaces}%       목각(B8F1B0A2)
%\def\mokgak{\hfontfamily{mg}}%
\def\^^b0{\@ifnextchar^^ed\only@gt\ga@or@gwa}
\def\only@gt#1#2#3{%
  \ifx#1^^ed\gtfamily\fi\ignorespaces}%                         고딕(B0EDB5F1)
\def\ga@or@gwa#1{%
  \ifx#1^^a1{\@josa{가}{이}}\else%        가(B0A1)
  \ifx#1^^fa{\@josa{와}{과}}\fi\fi}%      과(B0FA)
\def\^^b1{\@ifnextchar^^c3\gs@or@gh\only@gr}
%\def\gs@or@gh#1#2#3#4#5{%
%  \ifx#2^^bc\hfontfamily{gs}#4#5\else%    궁서(B1C3BCAD)
%  \hfontfamily{gh}\fi\ignorespaces}%      궁흘림(B1C3C8EAB8B2)
\def\only@gr#1#2#3#4#5{%
  \ifx#1^^d7\hfontfamily{gr}\fi\ignorespaces}% 그래픽(B1D7B7A1C7C8)
%
%\def\새명조{\hfontfamily{sm}\ignorespaces}% 새명조(BBF5B8EDC1B6)
%%\def\필기{\hfontfamily{pg}\ignorespaces}%   필기  (C7CAB1E2)
%\def\필기{%
%  \@ifnextchar a{\hfontfamily{pga}\@gobble}{\hfontfamily{pg}\ignorespaces}} 
%\def\펜#1#2#3#4{\ifx#1^^c8\hfontfamily{ph}% 펜흘림(C6E6C8EAB8B2)
%  \else\hfontfamily{pn}\fi\ignorespaces}%   펜글씨(C6E6B1DBBEBE)
%\def\봄글씨{\hfontfamily{bm}\ignorespaces}% 봄글씨(BABDB1DBBEBE)
\def\타자{\hfontfamily{tz}\ignorespaces}%   타자  (C5B8C0DA)
%\def\신문{\hfontfamily{sh}\ignorespaces}%   신문  (BDC5B9AE)
%\def\바다{\hfontfamily{vd}\ignorespaces}%   바다  (B9D9B4D9)
%\def\디나루{\hfontfamily{dn}\ignorespaces}% 디나루 (B5EFB3AAB7E7) 
%%%%% hangul 1.0 \ㅣ, \ㅡ compatibility.
\def\^^a4{%
	\@ifnextchar^^d1{\f@urI@}{\f@urEU@}%
}
\def\f@urI@^^d1{\으}
\def\f@urEU@^^d3#1#2{\@josa{#1#2}{이#1#2}}

%%% dautojosa 스타일 명령
%% \fjs 명령
\DeclareRobustCommand*{\DEFINEJOSA}[1]{\texorpdfstring{#1\xdef\make@josa{#1}}{#1}}
\def\Jaso#1{\DEFINEJOSA{\jaso{#1}}}
\def\PJaso#1{\DEFINEJOSA{\pjaso{#1}}}
\def\OJaso#1{\DEFINEJOSA{\ojaso{#1}}}
\def\Gana#1{\DEFINEJOSA{\gana{#1}}}
\def\PGana#1{\DEFINEJOSA{\pgana{#1}}}
\def\OGana#1{\DEFINEJOSA{\ogana{#1}}}
\def\ONum#1{\DEFINEJOSA{\onum{#1}}}
\def\PNum#1{\DEFINEJOSA{\pnum{#1}}}
\def\HNUM#1{\DEFINEJOSA{\hnum{#1}}}
\def\PEng#1{\DEFINEJOSA{\peng{#1}}}
\def\OEng#1{\DEFINEJOSA{\oeng{#1}}}
%% arabic, roman... etc.
\def\HArabic#1{\DEFINEJOSA{\arabic{#1}}}
\def\HAlph#1{\DEFINEJOSA{\Alph{#1}}}
\def\Halph#1{\DEFINEJOSA{\alph{#1}}}
\def\HROMAN#1{\DEFINEJOSA{\hRoman{#1}}}
\def\Hroman#1{\DEFINEJOSA{\hroman{#1}}}
%%
\def\jong{3}
\def\jung{2}
\def\rieul{1}
\DeclareRobustCommand*{\fjs}[1]{\texorpdfstring{\xdef\make@josa{#1}}{#1}}
%% xjf, DEFINEJOSA
\def\xjs#1{\DEFINEJOSA{#1}}
\newcommand\PageName{\DEFINEJOSA{페이지}}
\providecommand\AltPageName{\DEFINEJOSA{쪽}}

%%% 드러냄표 (2005/04/10 koaunghi@kornet.net)
\def\circemph@size#1{\leavevmode%
  \setbox0\hbox{\fontencoding{OT1}\fontseries{m}\selectfont!}%
  \dimen@\ht0\advance\dimen@-.3ex%
  \rlap{\raise.7\dimen@\hbox{\fontencoding{OT1}\fontseries{m}\selectfont\rule{.3\dimen@}{0pt}\char'27}}#1}
\def\dotemph@size#1{\leavevmode%
  \setbox0\hbox{\fontencoding{OT1}\fontseries{m}\selectfont!}%
  \dimen@\ht0\advance\dimen@-.3ex%
  \rlap{\raise.7\dimen@\hbox{\fontencoding{OT1}\fontseries{m}\selectfont\rule{.7\dimen@}{0pt}\char'137}}#1}

\def\circem{\let\hemph@size\circemph@size}
\def\dotem#1{\let\hemph@size\dotemph@size}
\def\circemph#1{{\let\hemph@size\circemph@size #1}}
\def\dotemph#1{{\let\hemph@size\dotemph@size #1}}


\endinput

%%% End of file `hfont.tex'.

